KRATOS: Multi-User Multi-Device-Aware Access Control System for the Smart Home

In a smart home system, multiple users have access to multiple devices, typically through a dedicated app installed on a mobile device. Traditional access control mechanisms consider one unique trusted user that controls the access to the devices. However, multi-user multi-device smart home settings pose fundamentally different challenges to traditional single-user systems. For instance, in a multi-user environment, users have conflicting, complex, and dynamically changing demands on multiple devices, which cannot be handled by traditional access control techniques. To address these challenges, in this paper, we introduce Kratos, a novel multiuser and multi-device-aware access control mechanism that allows smart home users to flexibly specify their access control demands. Kratos has three main components: user interaction module, backend server, and policy manager. Users can specify their desired access control settings using the interaction module which are translated into access control policies in the backend server. The policy manager analyzes these policies and initiates negotiation between users to resolve conflicting demands and generates final policies. We implemented Kratos and evaluated its performance on real smart home deployments featuring multi-user scenarios with a rich set of configurations (309 different policies including 213 demand conflicts and 24 restriction policies). These configurations included five different threats associated with access control mechanisms. Our extensive evaluations show that Kratos is very effective in resolving conflicting access control demands with minimal overhead and robust against different attacks.

==> policy_negotiator.tex <==
%Berkay: passed
\section{Policy Negotiation and Execution Engine} 
\label{task:negengine}
For policy negotiation and execution, \projectname considers three essential research questions: (1) How does \projectname handle the policy conflicts between users with the same and different priority levels?, (2) How does \projectname handle restriction policies without affecting smart home operations?, and (3) How are the generated policies executed in a multi-user smart home environment? In the following, we address these questions.

%Berkay passed.
\subsection{Policy Negotiation Process}
Access control in a multi-device multi-user smart home system is governed by compiling and negotiating all users' demands and restrictions expressed in user policies. Both \textit{demand} and \textit{restrict} clauses state conditions and imply opposing actions. Indeed, user policies might include \textit{soft} and \textit{hard} conflicts. The soft conflicts are used to define conflicts with overlapping acceptable conditions between users with same or different priorities. As an example, Alice and Gary have different user priorities and desires two different policies on a smart thermostat, such as \textit{Alice demands temperature in 65-75 degree range} and \textit{Bob demands 70-80 degree range}. \projectname flags the desires of the users as a soft conflict.
On the other hand, hard conflicts occur when two users with the same priority level desire policies with no overlapping conditions. For instance, Alice and Bob have the same priority over the temperature values of 60-70 and 75-85. \projectname flags this type of desires as hard conflicts. Furthermore, a demand clause results in a hard conflict on restrict clause if conditions have any overlap in user-device pairs. Lastly, conflicting clauses between users from different authorities, roles, classes (e.g., child-mother, a regular resident vs. a rare visitor) lead to hard authority conflicts.  

%Berkay passed.
The \textit{Negotiation Engine} will process all the policies and compute the negotiated result. It first models the users' authorities (classes, roles) in a multi-layer list.  Figure~\ref{fig:authoritylist} illustrates this model. User authorities are split into ordered classes. Class 0 has the highest authority, and a higher class number means a lower priority. Each class may include a list of users (or roles as roles are just a set of users). Users at the same priority class shares the same authority. \projectname considers four types of conflicts between user policies after users are classified into authorities.
%Berkay passed.
In this, each policy clause is compiled into a quintuple, $\Psi =  \{P,U,D,\mathcal{C},A\}$, where $P$ is the policy owner (that shows who states this clause), $U$ is the target user (about whom this statement is), $D$ is the smart device subjected,  $\mathcal{C}$ is a set of conditions over $D$ and $U$, and configurable environmental attributes, and finally $\mathcal{A}\in\{demand,restrict\}$ is the action requested by this statement when the set of conditions are satisfied. \projectname implements an algorithm to solve the policy conflicts through a set of equations as follows:

%Berkay: would be nice if we can align these left
\begin{equation}
\footnotesize
\begin{split}
\begin{aligned}
interfere(\Psi_i,\Psi_j) \gets  U_i = U_j \land D_i = D_j
\end{aligned}
\end{split}
\end{equation}
\begin{equation}
\footnotesize
\begin{split}
\begin{aligned}
hard\_conflict(\Psi_i,\Psi_j) \gets interfere(\Psi_i,\Psi_j) \land ( \\
    (A_i \neq A_j  ~\land \forall c \in \mathcal{C}_i \cap \mathcal{C}_j :  \Theta(\mathcal{V}(c,\mathcal{C}_i), \mathcal{V}(c,\mathcal{C}_j) ) ) \\ % there exists X, x in \mathcal{C}_i and x in \mathcal{C}_j 
    \lor ( A_i = A_j  ~\land \exists c \in \mathcal{C}_i \cap \mathcal{C}_j :  \neg \Theta(\mathcal{V}(c,\mathcal{C}_i), \mathcal{V}(c,\mathcal{C}_j) ) )   % there exists X, x in \mathcal{C}_i and x in \mathcal{C}_j 
) \\ % there is overlap at contradicting actions or there is no overlap at similar actions.
\end{aligned}
\end{split}
\end{equation}
\begin{equation}
\footnotesize
\begin{split}
\begin{aligned}
soft\_conflict(\Psi_i,\Psi_j) \gets interfere(\Psi_i,\Psi_j) \land ( \\
    (A_i = A_j  ~\land \forall c \in \mathcal{C}_i \cap \mathcal{C}_j :  \Theta(\mathcal{V}(c,\mathcal{C}_i), \mathcal{V}(c,\mathcal{C}_j) ) ) \\ % for the same action, there should be overlapping region for all conditionals
    \lor ( A_i \neq  A_j  ~\land \exists c \in \mathcal{C}_i \cap \mathcal{C}_j : \mathcal{V}(c,\mathcal{C}_i) \neq \mathcal{V}(c,\mathcal{C}_j) )   % for opposite actions, there should be at least one non-overlapping region for a conditional.  
) % there is overlap at contradictin actins or there is no overlap at similar actions.
\end{aligned}
\end{split}
\end{equation}
\begin{equation}
\footnotesize
\begin{split}
\begin{aligned}
HAC(\Psi_i,   \Psi_j)  \gets  hard\_conflict(\Psi_i,\Psi_j) \land \Xi(P_i) \neq \Xi(P_i) 
\end{aligned}
\end{split}
\end{equation}
\begin{equation}
\footnotesize
\begin{split}
\begin{aligned}
SAC  (\Psi_i,   \Psi_j)   \gets  soft\_conflict(\Psi_i,\Psi_j) \land \Xi(P_i) \neq \Xi(P_i)
\end{aligned}
\end{split}
\end{equation}
\begin{equation}
\footnotesize
\begin{split}
\begin{aligned}
HCC  (\Psi_i,    \Psi_j)   \gets  hard\_conflict(\Psi_i,\Psi_j) \land \Xi(P_i) = \Xi(P_i)
\end{aligned}
\end{split}
\end{equation}
\begin{equation}
\footnotesize
\begin{split}
\begin{aligned}
SCC  (\Psi_i,    \Psi_j)   \gets  soft\_conflict(\Psi_i,\Psi_j) \land \Xi(P_i) = \Xi(P_i)
\end{aligned}
\end{split}
\end{equation}

 \begin{figure*}[h!]
 \centering
 \small
\begin{equation}
 \centering
        \mathcal{N}(\Psi_i,\Psi_j)= 
\begin{cases}
 \centering
    \begin{cases} 
        \Psi_i & \text{if } \Xi(P_i) > \Xi(P_i) \\
         \Psi_j & \text{otherwise}
    \end{cases},&   \text{if } HAC(\Psi_i,\Psi_j) \\
    \begin{cases} 
        \{P_i \cup P_j,U_i,D_i,\mathcal{C}_i \cup \mathcal{C}_j,A_i\} & \text{if } A_i = A_i \\
         \{P_i \cup P_j,U_i,D_i,\mathcal{C}_i \cup \neg \mathcal{C}_j,A_i\} & \text{otherwise}
    \end{cases},&   \text{if } SAC(\Psi_i,\Psi_j) \\
    \begin{cases} 
        majority\_vote(\Psi_i,\Psi_j)  & \text{if } binary(D_i) \\
        arbitrate(\Psi_i,\Psi_j) & \text{otherwise}
    \end{cases},&   \text{if } HCC(\Psi_i,\Psi_j) \\
    \begin{cases} 
        \{P_i \cup P_j,U_i,D_i,\mathcal{C}_i \cup \mathcal{C}_j,A_i\} & \text{if } A_i = A_i \\
         \{P_i \cup P_j,U_i,D_i,\mathcal{C}_i \cup \neg \mathcal{C}_j,A_i\} & \text{otherwise}
    \end{cases},&   \text{if } SCC(\Psi_i,\Psi_j) \\
\end{cases} \label{eq:nagotiation}
\end{equation}
%\vspace{-10pt}}
\caption{ Negotiation algorithms to resolve conflicts where 
 HAC is hard authority conflict, SAC is soft authority conflict, 
 HCC is hard competition conflict, 
 and SCC is soft competition conflict.
 }
 \vspace{-0.2cm}
\end{figure*}

%Berkay passed.
\noindent where $\Psi_i,\Psi_j$ is the evaluated pair of policies, and  $\mathcal{V}(c,C)$ is the value function that returns the value of conditional $c$ in the set $C$, $\Theta(x,y)$ checks the overlap between the provided $(x,y)$ tuple and $\Xi(u)$ returns the authority of user $u$ as the value of user's assigned priority class.

%Berkay passed.
When two different policies include clauses of the same user's access for the same device, there can be an \textit{interference} between those clauses. Any such possible interference is further checked to disclose the potential conflicts. In this, \textit{hard conflicts} can happen when two interfering clauses dictate different actions for some overlapping cases or dictate the same action for never overlapping cased. In other words, when policies have no possible way of cooperation or compromising, (e.g., Alice demands 60-70 range while Bob demands of 75-85 range for the same thermostat). In such cases, \projectname detects a  \textit{hard conflict}; however, if the same action exists with some common overlap while opposite actions never occur together, such interference is a \textit{soft conflict}. Moreover, conflicts are further categorized as \textit{Authority Conflicts} or \textit{Competition Conflicts} based on the authority of policy owners. When two conflicts happen between users' policies who have different authority classes, \projectname defines an \textit{authority conflict}. However, if the users have the same authority, \textit{competition conflicts} happens. By incorporating these with hard and soft conflicts, \projectname overall implements four distinct conflict types. As such, the negotiation $\mathcal{N}$ between two given policy clauses $(\Psi_i,\Psi_j)$ can be formally expressed and computed by a sample function as in Equation~\ref{eq:nagotiation}. 
%
%Berkay passed. The sentence below comes from nowhere.
Here, as an example, in the case of a hard authority conflict (e.g., mother vs. child with contradicting clauses) result is the clause of the user with the higher authority (e.g., mother). On the other hand, in the case of both soft authority and soft competition conflicts, the result of the negotiation is a new clause with common features. 

%ground 

% Meanwhile, we define any smart device service with two possible values as binary (e.g., a smart switch with on-off states) otherwise as ranged (e.g., a thermostat with a valid value range). Then, when a hard competition conflict is 
% encountered, the negotiation process 
% check if the subjected device service is binary.
% If so, the negation process is resolved by employing a majority voting scheme (i.e., the most frequently asked value). If the smart device's  service accepts ranged values, the negotiated policy is computed by arbitrating the policy value. For instance, the average of requested values is the negotiation result. 


%
% $\mathcal{N}(\Psi_i,\Psi_j)$ 
%
% Hard Conflicts are 
%
% Hard Authority Conflict
% Soft Authority Conflict
% Hard Competition Conflict
% Soft Competition Conflict
% Competition/Racing
% Devices attribute: Binary states, partial states. 
% Users attribute:  priority classes
%



%Hence, we investigate different  algorithms to extend this basic pair-wise negotiation construct (Equation~\ref{eq:nagotiation}) for a set of policies. Extreme %Edge 
%cases like resolving a tie in the majority voting will also be studied. Further negotiation algorithms for different device service characteristics %SU exemplify here pls . DONE
% will also be researched. 
 %new, please revise.
% For example, devices might have services that accept different type of variables such as ranges of continuous data (e.g., [50,100]), or discrete values (e.g., 10, 50, or 100), or categorical (non-numeric) values (e.g., weekdays or weekend). In the negotiation process,  % including 
% these types of data, accordingly, mean, median, mode, and other types of central tendency measures will be considered as candidate negotiation functions. 

%\vspace{-20pt}

%Berkay: equations needs fix. Does not look good.
\subsubsection{Access Control Rule Generation} \label{task:rulegen}

\begin{figure}[t!]%{r}{0.48\textwidth}
\vspace{-0.3cm}
\centering
 %\resizebox{\columnwidth}{!}
\begin{footnotesize}
 \begin{align*}  
   ABAC(\Psi_i) \coloneqq \{B \mid  & \operatorname{action}(B) = \operatorname{A_i} \land \\ &
   \operatorname{subject}(B) = \operatorname{U_i} \land \\  &
   \operatorname{resources}(B) = \operatorname{D_i} \land \\  &
\operatorname{constraints}(B) = \operatorname{T_{\mathcal{C}_i}}   \} \\
{ \text{where} } & \\
 T_C  \coloneqq\{ 
  c \mid & c \text{ satisfies the same} \\ & \text{conditions of C in mapped} \\ & \text{attributes into ABAC policy} \} 
 \end{align*}
\end{footnotesize} 
\vspace{-10pt}
\footnotesize
\caption{An example of mapping a sample policy to ABAC rule through a transformation function. $ABAC(\Psi_i)$ is a translation of action, subject, resources, constraints defined in a policy.
} 
\label{fig:rulegen}
\vspace{-5pt}
\end{figure}

%Berkay passed
The negotiated policy computed in the previous section is converted into an enforceable access control rule. The negotiated policy clause, $\Psi =  \{P,U,D,\mathcal{C},A\}$, have a 5-tuple format  and indeed well suited for existing attribute-based access control (ABAC) systems.  Thus, \projectname uses an ABAC-like enforcement for the final rule generated. Here, the policy, $B$, is the set of \{action, subject, resource, constraints\} tuples for a negotiated smart home policy. As an example,  Figure~\ref{fig:rulegen} illustrates a simple example where $ABAC(\Psi_i)$  holds a direct translation of actions, subjects, resources, and constraints. We develop an ABAC-like rule generator that enforces the rules in a control device. The generator is integrated into the hub device as a unified enforcement point. 


%To give an idea about the mapping relation,  
% transformed constraints of condition set~$C$. %SU translation into what?  
% The suitability of ABAC %paradigm 
% for the smart home domain will be investigated and a representative rule generation and enforcement system will be developed. 
% \vspace{-10pt}
%SU I think we should not use ABAC word specifically, otherwise the readers will attack saying what is novel ;) 
%SU made all these plural because there may be more than one subject and actions in the outcome? or am I missing something?. Fixed. this is a single rule. each subject-resource pair is handled in a different rule.

%berkay passed.
\subsection{Policy Execution Process}
\label{patch}
Policy execution enforces the final policies generated from the policy negotiation process. Smart home devices can be controlled through a mobile phone controller app or by installing different device-specific apps in the system (e.g., Samsung SmartThings). Policy execution process appends the generated policies in the smartphone controller app or the installed smart home apps. To append the policies, \projectname adds conditional statements to the app source code to enforce the policies. When a user tries to change the state of the device, the app asks policy execution engine to check in the policy table generated by a policy generator. If an acceptable condition is matched, the policy execution engine returns the policy to the app and creates a binary decision (true for the accepted policy and false for the restricted policy) in the conditional branches. Based on the decision enforced by the policy execution engine, the user command in a smart home app is executed. A sample patched app is presented in Appendix~\ref{patch}.
